Beyond Masking: Demystifying Token-Based Pre-Training for Vision Transformers

The past year has witnessed a rapid development of masked image modeling (MIM). MIM is mostly built upon the vision transformers, which suggests that self-supervised visual representations can be done by masking input image parts while requiring the target model to recover the missing contents. MIM has demonstrated promising results on downstream tasks, yet we are interested in whether there exist other effective ways to `learn by recovering missing contents'. In this paper, we investigate this topic by designing five other learning objectives that follow the same procedure as MIM but degrade the input image in different ways. With extensive experiments, we manage to summarize a few design principles for token-based pre-training of vision transformers. In particular, the best practice is obtained by keeping the original image style and enriching spatial masking with spatial misalignment -- this design achieves superior performance over MIM in a series of downstream recognition tasks without extra computational cost. The code is available at https://github.com/sunsmarterjie/beyond_masking.

==> backup.tex <==
%%% 1. table

\begin{table}[!t]
\centering
\fontsize{9.5}{11.0}\selectfont
%\setlength{\tabcolsep}{1.2mm}
\setlength{\tabcolsep}{2.0mm}
% \setlength{\tabrsep}{2.0mm}
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
{} & \multicolumn{3}{c|}{\textbf{Factors}} & \multicolumn{3}{c|}{\textbf{ImageNet-1K}} & \multicolumn{3}{c}{\textbf{COCO/ADE20K}} \\
\textbf{Task} & PTD  & MPI  & SMA  & FT & LP  & NP & OD & IS & SS \\ \midrule
\textit{None}  & --   & --  & --  & 80.7  & 4.1 & 00.0 & 00.0 & 00.0 & 00.0 \\ \midrule
%\multirow{2}{*}{Task} & \multirow{2}{*}{\stackbox[c][c]{information \\ lost}}  & \multirow{2}{*}{distribution \\ hold}  & \multirow{2}{*}{spatial\\ change} & \multirow{2}{*}{Acc.} \\  \midrule
MoCo-v3$^\dagger$  &--  &--  &--  &83.0  &76.2 & -- & 45.5 & 40.5 & -- \\
DINO$^\dagger$   &--  &--  &--  &83.3  &77.3  & -- & 46.8 & 41.5 & 00.0 \\ \midrule
BEiT  &--  &--  &--  &83.0  &\textcolor{red}{37.6} & -- & 39.5 & 35.9 & 00.0 \\
(m) MAE~\cite{MAE}  & \textcolor{blue}{\textbf{Y}}  & \textcolor{blue}{\textbf{Y}} & \textcolor{red}{\textbf{N}} & 82.9  &61.5  &63.3 & 00.0 & 00.0 & 00.0 \\ \midrule
(a) distorted   & \textcolor{magenta}{\textbf{P}}  & \textcolor{magenta}{\textbf{P}} & \textcolor{blue}{\textbf{Y}} & 82.5   & 60.7 & 62.4 & 00.0 & 00.0 & 00.0  \\
(b) zoomed-in     & \textcolor{blue}{\textbf{Y}} & \textcolor{blue}{\textbf{Y}} & \textcolor{blue}{\textbf{Y}} & 82.5   & 61.0 & 62.6 & 00.0 & 00.0 & 00.0  \\
(c) zoomed-out    & \textcolor{blue}{\textbf{Y}} & \textcolor{red}{\textbf{N}} & \textcolor{blue}{\textbf{Y}} & 82.2   & 59.0 & 60.6 & 00.0 & 00.0 & 00.0  \\ 
(d) blurred      & \textcolor{red}{\textbf{N}} & \textcolor{magenta}{\textbf{P}} & \textcolor{red}{\textbf{N}} & 81.8   & 55.3 & 57.2 & 00.0 & 00.0 & 00.0  \\ 
(e) de-colorized   & \textcolor{red}{\textbf{N}} & \textcolor{magenta}{\textbf{P}} & \textcolor{red}{\textbf{N}} & 81.2  & 55.6 & 57.9 & 00.0 & 00.0 & 00.0  \\
\bottomrule
\end{tabular}
\caption{The downstream recognition performance of the ViT-base model pre-trained for $300$ epochs with different learning objectives (DINO trained for $400$ epochs). In the left-hand part, \textit{None} means no pre-training is used, and $^\dagger$ indicates \textcolor{red}{xxxxxxxxx}. In the middle part, we list three important aspects of the learning objectives, including preserving the token-level data distribution (PTD), missing partial information (MPI), and spatial misalignment (SMA), and \textcolor{blue}{\textbf{Y}}, \textcolor{magenta}{\textbf{P}}, \textcolor{red}{\textbf{N}} denote \textcolor{blue}{\textbf{yes}}, \textcolor{magenta}{\textbf{partly yes}}, and \textcolor{red}{\textbf{no}}, respectively. In the right-hand part, we list the accuracy on ImageNet under different evaluation protocols (including fine-tuning -- FT, linear probing -- LP, non-linear probing -- NP) as well as the accuracy on MS-COCO object detection (OD) and instance segmentation (IS) and ADE20K semantic segmentation (SS). Please refer to the main text for further analysis. OD and IS are measured by mean AP, and SS is measured by mean IOU.}
\label{tab:recognition}
\end{table}




%%% 2. analysis

First, we observe that, a bit surprisingly, the effectiveness of pre-training is not entirely related to the difficulty of the learning objective. In particular, there is no difficulty at all to recover the original image from its zoomed-out copy\footnote{This is not related to super-resolution, as the final training loss is \textcolor{red}{just comparable to} that of directly scaling up with bilinear interpolation.}, while colorizing a grayscale image requires semantic understanding~\cite{?,?}; however, the former task works much better than the latter.

Second, to understand how the learning algorithm works, we extract three factors from the pre-training objectives, including (i) whether the token-level data distribution is preserved\footnote{Definition: the input only contains patches that can be sampled from the dataset using regular transformations (\textit{e.g.}, rescaling, cropping, \textit{etc.}) -- note that a large part of the distorted patches are normal, but all patches of a blurred image or a de-colorized image are not.}, (ii) whether partial image contents are missing from the input, and (iii) whether a pair of input and output tokens at the same position may be misaligned (\textit{i.e.}, they correspond to different image regions). We provide detailed analysis below.
\begin{enumerate}
\item We point out that (i) is a fundamental requirement -- we conjecture that (d) and (e) produce inferior performance because they fail to conform it. To further validate this point, we perform diagnostic studies using the zoomed-out input, but fill up the empty region using either dummy patches (\textit{i.e.}, all pixels are black) or patches from other images. According to the results shown in Table~\ref{?}, a significant accuracy drop is observed, implying that token-level pre-training is sensitive to data distribution\footnote{\textcolor{red}{One may think that such modifications have reduced the difficulty of the learning objective, but we point out that the target model, being a vision transformer, processes each patch individually (except for the self-attention mechanism). Therefore, in the second situation (patches are copied from other images), we conjecture that the issue lies in data distribution rather than difficulty.}}.
\item Given that (i) is satisfied, both (ii) and (iii) are helpful to pre-training, because the target model must learn to predict something, either the missing contents, or the correct position of the visible contents. Indeed, according to the comparison among (m)(a)(c), we find that (ii) is stronger than (iii), and we conjecture the reason to be that (iii) still brings a gap between the pre-training and fine-tuning stages (\textit{i.e.}, the pre-training stage always receives incorrect position embeddings).
\item Continuing with spatial misalignment, we design another task that randomly shuffles the input patches and requires the target model to recover the original image. Note that this is different from solving jigsaw puzzles~\cite{?,?} because the goal is to pixel-wise recover the original image rather than predicting the correct ID of input patches. With this proxy, the pre-trained model achieves a $82.?\%$ accuracy under the fine-tuning protocol, which is comparable to others. This may be an interesting topic that worths further investigation.
\item Finally, we emphasize that the three factors do not cover all necessary conditions that improve token-level pre-training. For example, as discussed in MAE~\cite{?}, the spatial distribution of masked patches impacts the pre-training performance, but the designed tasks involving spatial information missing (\textit{i.e.}, (a)(c)) belong to the so-called `blocked' masking style, which was shown to produce weaker recognition results~\cite{mae}.
\end{enumerate}


%%% 3. ablation

\subsection{Diagnostic Studies}
\label{experiments:diagnosis}

We first investigate some important hyper-parameters of the pre-training tasks. The results are summarized in Table~\ref{tab:diagnosis}. For all tasks except (e), the best performance is obtained under a proper difficulty. The same trend was also observed in MAE~\cite{mae} where an intermediate masking ratio (\textit{e.g.}, $75\%$) is the overall best choice. This phenomenon aligns with our finding that preserving token-level data distribution is a fundamental condition of pre-training -- with an over-high difficulty, the gap between the distributions of upstream and downstream data becomes significant and thus harms the recognition accuracy.

To enhance the understanding, we further create some variants based on the task of recovering zoomed-out images. Recall that we force the border of the zoomed-out image to be exactly on the border between neighboring tokens, and we fill up the outer region with patches from the same image. Based on the best option ($S=160$, see Table~\ref{tab:diagnosis}), violating either condition\footnote{To violate the second condition, we fill up the outer region with all-black blocks or patches copied from other images, which produce similar performance.} causes the fine-tuning accuracy to drop from $82.2\%$ to $8?.?\%$ and $8?.?$, respectively.

\subsection{Rethinking Studies: clear this part ...}

\textcolor{red}{We design 2-3 ablation experiments for task (a), (b) and (c) except (d) and (e) because of their poor performances. All the models are trained for $300$ epochs, and the results denote finetuning scores.}

\textcolor{red}{For task (a), we design $2$ settings. Firstly, to guarantee there is no missing pixels for input compared to output, we distorted a $256\times256$ cropped image, and predict the center $224\times224$ part. The distorted image is resized into $224\times224$ before put into transformer. The result is $82.1\%$, just slightly lower than $82.5\%$, which illustrates that the improvement of task (a) comes from the distortion operation but not pixel lost. Secondly, we use a easy distorted transformation - horizontal wave distortion, which does not lead to pixel missing. Interestingly, we also achieve a good result of $81.9\%$, which further verified that recovering distorted image is able to improve self-supervised transformer.}

\textcolor{red}{For task (b), we also propose $2$ settings to test zoom-in. Firstly, we randomly crop a $160\times160$ part on the original image instead of picking in the center of the image. The performance drops from $82.5\%$ to $81.5\%$ straightly. Randomly cropping the center part as input makes the task unpredictable, which confuses the transformer to predict how long the range is. This also indicates that predicting the missing pixel does not always work. Secondly, we use MAE pipeline to reserve the inter $160\times160$ part and predict the outer patches. This setting leads to the result of $82.3\%$, which implies misalignment is helpful for training self-supervised vision transformers.}

\textcolor{red}{For task (c), we add $3$ interesting experiments. We first only zoom-out the original image to $160\times160$ without padding the edges. This gets a poor performance of $79.9\%$. Then, we randomly pad the edges using black patches and patches from other images. These setting cause $80.0\%$ and $80.5\%$ respectively. All these $3$ settings make the recovering task easy: the first only requires the model to learn the ability of magnify, which is irrespective of semantics; the last two make the input have the clear boundaries. }

\te\textcolor{red}{Above ablation studies further verify our conclusion: xxx}



%%% x. timetable



\iffalse
\section{\textcolor{red}{TODO list}}

Timetable as of Feb 14th

\begin{itemize}
\item Combining multiple objectives -- due 02.21 \\
(1) dual-branch results \\
(2) directly combining spatial misalignment and masking???
\item Story to be discussed and rewritten -- due 02.21 \\
(1) masking is NOT the only objective that works \\
(2) spatial misalignment also works \\
(3) any clues for `warming-up'? -- linear/non-linear tests (for both token-level and image-level pre-training!)
\item Large-scale experiments and large-scale tests \\
(1) detection and segmentation -- due 02.18 \\
(2) ViT-large experiments -- due 02.25
\item Proofreading \\
(1) sent to other mentors, e.g. Xiaopeng \\
(2) presentation at seminar -- scheduled at 02.24 \\
(3) sent to other people, e.g. Prof Ye & Tian
\end{itemize}

\textcolor{red}{OUTDATED}

Timetable as of Jan 20th -- mark finished terms with \textcolor{blue}{blue}, and delayed terms with \textcolor{red}{red}

\begin{itemize}
\item Week 1 due Jan 24 \\
\textcolor{blue}{1. Confirm 5 pretext tasks + masked image modeling -- any more tasks? This can be done by considering possible combinations of the factors to be diagnosed.}\\
2. Paper draft with the framework clear. \\
3. Experiment plans confirmed, in particular:\textcolor{blue}{(1) Shall we combine some of the tests for better results? Combining them with masked image modeling may be required; }(2) Do we need other tests, such as \textcolor{blue}{linear probing, fine-tuning with more epochs,} fine-tuning on object detection, etc.? \textcolor{blue}{and finetune on segmentation.}
\item Week 2 due Jan 31 \\
\textcolor{blue}{1. Confirm the best parameters for individual experiments (not changed hereafter).} \\
\textcolor{red}{2. Test the best parameters with combined experiments.}
\item Week 3 due Feb 7 \\
1. Finish the combined experiments (construct and complete the table of Sec 2.3), with the estimation of marginal effects. \\
2. Plan (and start if possible) large-scale experiments (ViT-L, ViT-base with 400+ epochs) and downstream tests (linear probing, detection, etc.).
\item Week 4 due Feb 14 \\
1. Paper v1 -- abstract, introduction, related work, conclusions can be missing. \\
2. Large-scale experiments -- checkpoint 1, status and updated plan.
3. Downstream tests -- checkpoint 1, status and updated plan.
\item Week 5 due Feb 21 \\
1. Paper v2 -- all contents ready, possibly with missing numbers. \\
2. Presentation at seminar. \\
3. Large-scale experiments -- checkpoint 2, status and updated plan.
4. Downstream tests -- checkpoint 2, status and updated plan.
\item Week 6 due Feb 28 \\
1. Paper v3 (almost ready for submission) -- sent to 5+ people for proofreading. \\
2. Large-scale experiments -- checkpoint 3, done.
3. Downstream tests -- checkpoint 1, done.
\item Week 7 due Mar 7 (deadline: 3:59 am, Mar 8) \\
1. Paper submission
\end{itemize}
\fi

